A Substrate Scheduler for Compiling Arbitrary Fault-tolerant Graph States

Graph states are useful computational resources in quantum computing, particularly in measurement-based quantum computing models. However, compiling arbitrary graph states into executable form for fault-tolerant surface code execution and accurately estimating the compilation cost and the run-time resource cost remains an open problem. We introduce the Substrate Scheduler, a compiler module designed for fault-tolerant graph state compilation. The Substrate Scheduler aims to minimize the space-time volume cost of generating graph states. We show that Substrate Scheduler can efficiently compile graph states with thousands of vertices for "A Game of Surface Codes"-style patch-based surface code systems. Our results show that our module generates graph states with the lowest execution time complexity to date, achieving graph state generation time complexity that is at or below linear in the number of vertices and demonstrating specific types of graphs to have constant generation time complexity. Moreover, it provides a solid foundation for developing compilers that can handle a larger number of vertices, up to the millions or billions needed to accommodate a wide range of post-classical quantum computing applications.

==> framework.tex <==
\naphann{This will be combined into our approach section}

\magenta{
The general approach to creating graph states is to apply controlled-phase gates between qubits of adjacent vertices in the graph state~\cite{cabello_optimal_2011} which can be performed by two parity check measurements. 
It can be easily seen that in the worst case when all controlled-phase gates are performed sequentially, one would require $O(|E|)$ Tocks which for dense graph will scale on the order of $O(N^2)$.
For this reason, we opted for the approach of using parity check measurement to directly project the state into the eigenspace of each of the stabilizer generators.
In contrast to the controlled-phase gate approach, this will scale only on the order of $O(N)$ Tocks.
The goal of this approach is then to minimize and parallelize these stabilizer generator projections.
}



Figure \ref{Fig.Frame} summarizes the key components of the Substrate Scheduler. Substrate Scheduler uses the adjacency matrix as input, which theoretically allows it to process any graph state that is represented as an adjacency matrix. 

\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{img/chart.png}
\caption{Flow chart for Substrate Scheduler.}
\label{Fig.Frame}
\end{figure}



The first step in the process is to reduce the number of stabilizer generators that need to be implemented. This is achieved by initializing the qubits so that they are already stabilized by some stabilizer generators. The next step is to determine the optimal mapping of the qubits. We proposed a heuristic scheme that works well for certain types of graphs. After that, the Substrate Scheduler finds the optimal schedule for the stabilizer generators and minimizes the time cost by measuring as many stabilizers as possible. This results in an optimized schedule of stabilizers to be measured and logical qubit allocation, which can be combined with the default layout design and passed on to a fault-tolerant quantum computer (i.e.  logical qubits encoded by quantum error correction) to generate a fault-tolerant quantum graph state.

